Semi-Supervised Singing Voice Separation with Noisy Self-Training

Recent progress in singing voice separation has primarily focused on supervised deep learning methods. However, the scarcity of ground-truth data with clean musical sources has been a problem for long. Given a limited set of labeled data, we present a method to leverage a large volume of unlabeled data to improve the model's performance. Following the noisy self-training framework, we first train a teacher network on the small labeled dataset and infer pseudo-labels from the large corpus of unlabeled mixtures. Then, a larger student network is trained on combined ground-truth and self-labeled datasets. Empirical results show that the proposed self-training scheme, along with data augmentation methods, effectively leverage the large unlabeled corpus and obtain superior performance compared to supervised methods.

==> background.tex <==
\subsection{Semi-supervised Learning with Self-Training}
\label{ssec:background}

Self-training is a semi-supervised framework in which a pre-trained teacher model assigns pseudo-labels for unlabeled data and then a student model is trained with the self-labeled dataset. It has been applied in several applications such as image recognition \cite{selftrn_rec_noisy_2019} and automatic speech recognition \cite{selftrn_asr_noisy_2020}. Our approach follows the noisy self-training method where we investigate data augmentation methods on musical signal and evaluate how they affect the separation performance.
